Grover's Search-Inspired Quantum Reinforcement Learning for Massive MIMO User Scheduling

The efficient user scheduling policy in the massive Multiple Input Multiple Output (mMIMO) system remains a significant challenge in the field of 5G and Beyond 5G (B5G) due to its high computational complexity, scalability, and Channel State Information (CSI) overhead. This paper proposes a novel Grover's search-inspired Quantum Reinforcement Learning (QRL) framework for mMIMO user scheduling. The QRL agent can explore the exponentially large scheduling space effectively by applying Grover's search to the reinforcement learning process. The model is implemented using our designed quantum-gate-based circuit, which imitates the layered architecture of reinforcement learning, where quantum operations act as policy updates and decision-making units. Moreover, the simulation results demonstrate that the proposed method achieves proper convergence and significantly outperforms classical Convolutional Neural Networks (CNN) and Quantum Deep Learning (QDL) benchmarks.

==> IEEE_WCNC_QRL_for_Massive_MIMO_User_Scheduling/acro.tex <==
\begin{acronym}
\acro{B5G}{Beyond 5G}
\acro{TDMA}{Time Division Multiple Access}
\acro{FDMA}{Frequency Division Multiple Access}
\acro{MIMO}{Multiple Input Multiple Output}
\acro{mMIMO}{massive Multiple Input Multiple Output} % Note: document uses both MIMO and mMIMO
\acro{MU-mMIMO}{Multi-user Massive Multiple Input Multiple Output}
\acro{CSI}{Channel State Information}
\acro{CSIT}{Transmitter Channel State Information}
\acro{BS}{Base Station}
\acro{UT}{User Terminal}
\acro{AI}{Artificial Intelligence}
\acro{ML}{Machine Learning}
\acro{QNN}{Quantum Neural Networks}
\acro{QDL}{Quantum Deep Learning}
\acro{LoS}{Line of Sight}
\acro{NLoS}{Non Line-of-sight}
\acro{QoS}{Quality of Service}
\acro{WMMSE}{Weighted Minimum Mean Square Error}
\acro{DNN}{Deep Neural Networks} % Note: document uses DNN and DNNs
\acro{RL}{Reinforcement Learning}
\acro{DQN}{Deep Q-networks} % Note: document uses DQNS
\acro{PRO}{Policy Optimisation}
\acro{AWGN}{Additive White Gaussian Noise}
\acro{AoD}{Angle-of-departure}
\acro{DFT}{Discrete Fourier Transform}
\acro{ULA}{Uniform Linear Antenna Array}
\acro{NN}{Neural Networks} % Note: document uses NN and NNs
\acro{AP}{Access Point}
\acro{UE}{User Terminal}
\acro{SNR}{Signal-to-noise Ratio}
\acro{SINR}{Signal-to-interference-plus-noise Ratio}
\acro{SLNR}{Signal-to-leakage-plus-noise Ratio}
\acro{GPU}{Graphic Processing Unit}
\acro{PL}{Path Loss}
\acro{ANN}{Artificial Neural Networks} % Note: document uses ANN and ANNs
\acro{CNN}{Convolutional Neural Networks} % Note: document uses CNN and CNNs
\acro{GNN}{Graph Neural Networks} % Note: document uses GNNS
\acro{dB}{Decibel}
\acro{PF}{Proportional Fairness}
\acro{CNOT}{Controlled-NOT}
\acro{QRL}{Quantum Reinforcement Learning}
\end{acronym}
